Trainable Structure Tensors for Autonomous Baggage Threat Detection Under Extreme Occlusion

Detecting baggage threats is one of the most difficult tasks, even for expert officers. Many researchers have developed computer-aided screening systems to recognize these threats from the baggage X-ray scans. However, all of these frameworks are limited in identifying the contraband items under extreme occlusion. This paper presents a novel instance segmentation framework that utilizes trainable structure tensors to highlight the contours of the occluded and cluttered contraband items (by scanning multiple predominant orientations), while simultaneously suppressing the irrelevant baggage content. The proposed framework has been extensively tested on four publicly available X-ray datasets where it outperforms the state-of-the-art frameworks in terms of mean average precision scores. Furthermore, to the best of our knowledge, it is the only framework that has been validated on combined grayscale and colored scans obtained from four different types of X-ray scanners.

==> lib/packages.tex <==
\usepackage{lib/comment}
\usepackage{graphicx}
\usepackage{amsmath,amssymb} % define this before the line numbering.
\usepackage{color}
% \usepackage{todonotes}
% INITIAL SUBMISSION - The following two lines are NOT commented
% CAMERA READY - Comment OUT the following two lines
% \usepackage{lib/ruler}
% \usepackage[width=122mm,left=12mm,paperwidth=146mm,height=193mm,top=12mm,paperheight=217mm]{geometry}

% \usepackage{amssymb,amsthm}
\usepackage[inline]{enumitem}
\usepackage{multirow}
\usepackage[caption=false]{subfig}
\usepackage{array}
\usepackage{url}
\usepackage{algpseudocode}
\usepackage{algorithm}
\usepackage[most]{tcolorbox}
\usepackage{booktabs}
\usepackage{capt-of}
\usepackage{multicol}
\usepackage{cite}

\usepackage[backref, hidelinks]{hyperref}
% \usepackage{cite}
\linespread{0.90}
% INITIAL SUBMISSION - The following two lines are NOT commented
% CAMERA READY - Comment OUT the following two lines
\usepackage{lib/ruler}
\usepackage[width=122mm,left=12mm,paperwidth=146mm,height=193mm,top=12mm,paperheight=217mm]{geometry}

\renewcommand{\equationautorefname}{Eq.}
\def\sectionautorefname{Section}
\def\subsectionautorefname{\sectionautorefname}
\def\subsubsectionautorefname{\sectionautorefname}
\def\subfigureautorefname{\figureautorefname}
\def\propositionautorefname{Proposition}
\def\algorithmautorefname{Algorithm}

\algnewcommand{\Initialize}[1]{%
  \State \textbf{Initialize:}
  \Statex \hspace{\algorithmicindent} \parbox[t]{.8\linewidth}{\raggedright #1}
}
\algnewcommand{\Output}{\item[\textbf{Output:}]}
\algnewcommand{\Input}{\item[\textbf{Input:}]}

\DeclareGraphicsExtensions{.png,.PNG,.jpg}
\graphicspath{{../../PaperImages/},{img/}}


\newcommand{\X}{\color{red}X}
\newcommand{\V}{{\color{green}\checkmark}}
\newcommand{\e}{\textbf{e}}
\renewcommand{\a}{\textbf{a}}
\newcommand{\T}{\mathbb{T}}
\newcommand{\Tu}{\mathcal{T_U}}
\newcommand{\Tl}{\mathcal{T_L}}
\newcommand{\Tr}{\mathcal{T_R}}
\renewcommand{\H}{\mathcal{H}}
\newcommand{\R}{\mathcal{R}}

\definecolor{darkgreen}{rgb}{0 .7 0}
\newcommand{\NW}[1]{ {\color{blue}{#1}} }
\newcommand{\SA}[1]{ {\color{cyan}{#1}} }
\newcommand{\SK}[1]{ {\color{darkgreen}{#1}} }
\newcommand{\MB}[1]{ {\color{purple}{#1}} }
\newcommand{\RR}[1]{ {\color{red}{#1}} }
%\newcommand{\RR}[1]{{{\color{red}\bf\uppercase{***#1***}}}}
